Improved Image Captioning via Policy Gradient optimization of SPIDEr

Current image captioning methods are usually trained via (penalized) maximum likelihood estimation. However, the log-likelihood score of a caption does not correlate well with human assessments of quality. Standard syntactic evaluation metrics, such as BLEU, METEOR and ROUGE, are also not well correlated. The newer SPICE and CIDEr metrics are better correlated, but have traditionally been hard to optimize for. In this paper, we show how to use a policy gradient (PG) method to directly optimize a linear combination of SPICE and CIDEr (a combination we call SPIDEr): the SPICE score ensures our captions are semantically faithful to the image, while CIDEr score ensures our captions are syntactically fluent. The PG method we propose improves on the prior MIXER approach, by using Monte Carlo rollouts instead of mixing MLE training with PG. We show empirically that our algorithm leads to easier optimization and improved results compared to MIXER. Finally, we show that using our PG method we can optimize any of the metrics, including the proposed SPIDEr metric which results in image captions that are strongly preferred by human raters compared to captions generated by the same model but trained to optimize MLE or the COCO metrics.

==> Makefile <==
all: main

main:
	pdflatex main;
	bibtex main;
	pdflatex main;
	pdflatex main;

clean:
	${RM} *~; \
	${RM} *.log; \
	${RM} *.aux; \
	${RM} *.bbl; \
	${RM} *.blg; \
	${RM} main.dvi; \



==> ica_model.tex <==
\subsection{Adding visual tags}
\label{sec:tags}

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/ShowTellICA}
    \caption{Model architecture of attribute augmented model. 
      The tokens in green and yellow are
      respectively \texttt{BOS} (beginning of sequence) and \texttt{EOS}
      (end of sequence) tokens. At testing time, output from previous time
      step $g_{t-1}$ is used as input in lieu of $y_{t-1}$.}
    \label{fig:show_tell_ica}
\end{figure}


In this section, we describe a simple extension to the basic model from 
Section~\ref{sec:model}. 
In particular, we leverage
an in-house image tagging system,
which is trained on a large, but noisily labeled,
dataset called JFT (see \cite{Chollet2016} for details).
This system returns a vector of 
probability scores $\vp = \{p_0, p_1, ..., p_N\}$
for a set of $N=3,713$ classes, where $p_i \in [0, 1]$ indicates the
probability of presence of a visual attribute of class $i$ in the
image.
Typically 60--70 tags have a non-zero confidence score  for each image.
See Figure~\ref{fig:examples} for some example outputs from this system.
A high-level diagram of this architecture is shown in
Figure~\ref{fig:show_tell_ica}.

Given the visual tag score vector, we compute the input to
the decoder RNN at time $t$ by combining the scores from the tagger
with the  
previous word in the sequence as follows:

\be
\vx_t = \vT_w \vw_t  + \vT_p \vp 
\ee

where $\vw_t$ is the embedding of the $t$'th word,
$\vT_w \in \calR^{d_h \times d_w}$ maps the word embedding
to the RNN state space,
$\vp$ is the vector of tag probabilities,
and $\vT_p \in \calR^{d_h \times d_p}$ maps
from the $d_p=N$ tags to the RNN state space.
We shall call our model Show-Tell-Tag.

Our attribute augmented model is similar to LSTM-A\textsubscript{5},
recently introduced in \cite{Yao2016}. The main difference lies in the
choice of CNN (we used Inception-V3 as opposed to ResNet) as well as
the vocabulary of visual tags (we train on an internal dataset with 3k
noisy tags, whereas they use multi-instance learning to train a
classifier to predict the top 1k words in COCO).  
(See also \cite{Wu2016} for some related work on using visual tags for
image captioning.)

